Existence of generalized Busemann functions and Gibbs measures for random walks in random potentials

We establish the existence of generalized Busemann functions and Gibbs-Dobrushin-Landford-Ruelle measures for a general class of lattice random walks in random potential with finitely many admissible steps. This class encompasses directed polymers in random environments, first- and last-passage percolation, and elliptic random walks in both static and dynamic random environments in all dimensions and with minimal assumptions on the random potential.

==> macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Packages go here
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{amsmath,amsfonts, amsthm,amssymb,mathrsfs,enumitem}   %F: enumitem is better than enumerate
\usepackage[cmyk]{xcolor}
%%% types of  labels:  [label=(roman*)]  \arabic*  \alph*    also under \itemize can use different symbols to mark items

\RequirePackage[colorlinks,urlcolor=my-blue,linkcolor=my-red,citecolor=my-green]{hyperref}

\usepackage[numbers,comma,square,sort&compress]{natbib}
\usepackage{xargs}
\usepackage[colorinlistoftodos,prependcaption,textsize=footnotesize]{todonotes}
\usepackage{pdfcomment}
\usepackage{comment}
\usepackage{bm}
\usepackage{scalerel}    %%%%  used first for scaling \bullet  
\usepackage{stmaryrd}   %%%% for integer interval notation 
\usepackage{mathabx}   %% made \widecheck work  
\usepackage{hyphenat}
\usepackage[utf8]{inputenc}
%\usepackage[notref,notcite]{showkeys}
%%%%  2019-03-22 Timo moved showkeys into the latex file itself in order to toggle it for printing. 
\usepackage{caption}
\usepackage{subcaption}
\usepackage{a4wide}
\usepackage{accents}
\usepackage{tikz,tikz-3dplot}
\usetikzlibrary{arrows.meta,decorations.markings,shadings}
\usepackage{graphicx}
\usepackage{chngcntr}
\usepackage{float} %needed to fix the figures

\usepackage{rotating,centernot,cancel}    %% to manipulate symbols (Timo 2019-03-25) 
\usepackage{geometry}
\geometry{
	letterpaper,
	total={6.5in, 9in},
	left=1in,
	top=1in,
}





\numberwithin{figure}{section}
\numberwithin{equation}{section}

\RequirePackage{transparent}
\RequirePackage{color}
\definecolor{my-link}{rgb}{0.5,0.0,0.0}
\definecolor{my-blue}{rgb}{0.0,0.0,0.6}
\definecolor{my-red}{rgb}{0.5,0.0,0.0}
\definecolor{my-green}{rgb}{0.0,0.5,0.0}
\definecolor{nicos-red}{rgb}{0.75,0.0,0.0}
\definecolor{really-light-gray}{gray}{0.8}
\definecolor{darkgreen}{rgb}{0.0,0.5,0.0}
\definecolor{darkblue}{rgb}{0.0,0.0,0.3}
\definecolor{nicosred}{rgb}{0.65,0.1,0.1}
\definecolor{light-gray}{gray}{0.7}
\definecolor{sussexg}{rgb}{0,0.7,0.7}
\definecolor{sussexp}{rgb}{0.4,0,0.4}
\definecolor{nicos-red}{rgb}{0.75,0.0,0.0}
\definecolor{carmine}{rgb}{0.59, 0.0, 0.09}
\definecolor{dartmouthgreen}{rgb}{0.05, 0.5, 0.06}

\overfullrule=1mm

\newcommand{\bbA}{\mathbb{A}}
\newcommand{\bbB}{\mathbb{B}}
\newcommand{\bbC}{\mathbb{C}}
\newcommand{\bbD}{\mathbb{D}}
\newcommand{\bbE}{\mathbb{E}}
\newcommand{\bbF}{\mathbb{F}}
\newcommand{\bbG}{\mathbb{G}}
\newcommand{\bbH}{\mathbb{H}}
\newcommand{\bbI}{\mathbb{I}}
\newcommand{\bbJ}{\mathbb{J}}
\newcommand{\bbK}{\mathbb{K}}
\newcommand{\bbL}{\mathbb{L}}
\newcommand{\bbM}{\mathbb{M}}
\newcommand{\bbN}{\mathbb{N}}
\newcommand{\bbO}{\mathbb{O}}
\newcommand{\bbP}{\mathbb{P}}
\newcommand{\bbQ}{\mathbb{Q}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbS}{\mathbb{S}}
\newcommand{\bbT}{\mathbb{T}}
\newcommand{\bbU}{\mathbb{U}}
\newcommand{\bbV}{\mathbb{V}}
\newcommand{\bbW}{\mathbb{W}}
\newcommand{\bbX}{\mathbb{X}}
\newcommand{\bbY}{\mathbb{Y}}
\newcommand{\bbZ}{\mathbb{Z}}

%bold face
\newcommand{\bfA}{\mathbf{A}}
\newcommand{\bfB}{\mathbf{B}}
\newcommand{\bfC}{\mathbf{C}}
\newcommand{\bfD}{\mathbf{D}}
\newcommand{\bfE}{\mathbf{E}}
\newcommand{\bfF}{\mathbf{F}}
\newcommand{\bfG}{\mathbf{G}}
\newcommand{\bfH}{\mathbf{H}}
\newcommand{\bfI}{\mathbf{I}}
\newcommand{\bfJ}{\mathbf{J}}
\newcommand{\bfK}{\mathbf{K}}
\newcommand{\bfL}{\mathbf{L}}
\newcommand{\bfM}{\mathbf{M}}
\newcommand{\bfN}{\mathbf{N}}
\newcommand{\bfO}{\mathbf{O}}
\newcommand{\bfP}{\mathbf{P}}
\newcommand{\bfQ}{\mathbf{Q}}
\newcommand{\bfR}{\mathbf{R}}
\newcommand{\bfS}{\mathbf{S}}
\newcommand{\bfT}{\mathbf{T}}
\newcommand{\bfU}{\mathbf{U}}
\newcommand{\bfV}{\mathbf{V}}
\newcommand{\bfW}{\mathbf{W}}
\newcommand{\bfX}{\mathbf{X}}
\newcommand{\bfY}{\mathbf{Y}}
\newcommand{\bfZ}{\mathbf{Z}}

\newcommand{\bfa}{\mathbf{a}}
\newcommand{\bfb}{\mathbf{b}}
\newcommand{\bfc}{\mathbf{c}}
\newcommand{\bfd}{\mathbf{d}}
\newcommand{\bfe}{\mathbf{e}}
\newcommand{\bff}{\mathbf{f}}
\newcommand{\bfg}{\mathbf{g}}
\newcommand{\bfh}{\mathbf{h}}
\newcommand{\bfi}{\mathbf{i}}
\newcommand{\bfj}{\mathbf{j}}
\newcommand{\bfk}{\mathbf{k}}
\newcommand{\bfl}{\mathbf{l}}
\newcommand{\bfm}{\mathbf{m}}
\newcommand{\bfn}{\mathbf{n}}
\newcommand{\bfo}{\mathbf{o}}
\newcommand{\bfp}{\mathbf{p}}
\newcommand{\bfq}{\mathbf{q}}
\newcommand{\bfr}{\mathbf{r}}
\newcommand{\bfs}{\mathbf{s}}
\newcommand{\bft}{\mathbf{t}}
\newcommand{\bfu}{\mathbf{u}}
\newcommand{\bfv}{\mathbf{v}}
\newcommand{\bfw}{\mathbf{w}}
\newcommand{\bfx}{\mathbf{x}}
\newcommand{\bfy}{\mathbf{y}}
\newcommand{\bfz}{\mathbf{z}}


\newcommand{\mfa}{\mathfrak{a}}
\newcommand{\mfb}{\mathfrak{b}}
\newcommand{\mfc}{\mathfrak{c}}
\newcommand{\mfd}{\mathfrak{d}}
\newcommand{\mfe}{\mathfrak{e}}
\newcommand{\mff}{\mathfrak{f}}
\newcommand{\mfg}{\mathfrak{g}}
\newcommand{\mfh}{\mathfrak{h}}
\newcommand{\mfi}{\mathfrak{i}}
\newcommand{\mfj}{\mathfrak{j}}
\newcommand{\mfk}{\mathfrak{k}}
\newcommand{\mfl}{\mathfrak{l}}
\newcommand{\mfm}{\mathfrak{m}}
\newcommand{\mfn}{\mathfrak{n}}
\newcommand{\mfo}{\mathfrak{o}}
\newcommand{\mfp}{\mathfrak{p}}
\newcommand{\mfq}{\mathfrak{q}}
\newcommand{\mfr}{\mathfrak{r}}
\newcommand{\mfs}{\mathfrak{s}}
\newcommand{\mft}{\mathfrak{t}}
\newcommand{\mfu}{\mathfrak{u}}
\newcommand{\mfv}{\mathfrak{v}}
\newcommand{\mfw}{\mathfrak{w}}
\newcommand{\mfx}{\mathfrak{x}}
\newcommand{\mfy}{\mathfrak{y}}
\newcommand{\mfz}{\mathfrak{z}}


\newcommand{\mfG}{\mathfrak{G}}
\newcommand{\mfS}{\mathfrak{S}}

%script
\newcommand{\sA}{\mathcal{A}}
\newcommand{\sB}{\mathcal{B}}
\newcommand{\sC}{\mathcal{C}}
\newcommand{\sD}{\mathcal{D}}
\newcommand{\sE}{\mathcal{E}}
\newcommand{\sF}{\mathcal{F}}
\newcommand{\sG}{\mathcal{G}}
\newcommand{\sH}{\mathcal{H}}
\newcommand{\sI}{\mathcal{I}}
\newcommand{\sJ}{\mathcal{J}}
\newcommand{\sK}{\mathcal{K}}
\newcommand{\sL}{\mathcal{L}}
\newcommand{\sM}{\mathcal{M}}
\newcommand{\sN}{\mathcal{N}}
\newcommand{\sO}{\mathcal{O}}
\newcommand{\sP}{\mathcal{P}}
\newcommand{\sQ}{\mathcal{Q}}
\newcommand{\sR}{\mathcal{R}}
\newcommand{\sS}{\mathcal{S}}
\newcommand{\sT}{\mathcal{T}}
\newcommand{\sU}{\mathcal{U}}
\newcommand{\sV}{\mathcal{V}}
\newcommand{\sW}{\mathcal{W}}
\newcommand{\sX}{\mathcal{X}}
\newcommand{\sY}{\mathcal{Y}}
\newcommand{\sZ}{\mathcal{Z}}

\newcommand{\wt}{\widetilde}
\newcommand{\wtx}{\widetilde{x}}

\def\w{\omega}
\def\zero{\mathbf{0}}

\def\ri{\mathrm{ri\,}}
\providecommand{\abs}[1]{\vert#1\vert}
\newcommand{\fl}[1]{\lfloor{#1}\rfloor} 
\newcommand{\flint}[1]{[\![{#1}]\!]} 
\def\xip{\overline{\xi}}
\def\pxi{\overline{p}}

\renewcommand{\tilde}{\widetilde}

\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator{\Cov}{Cov}
\DeclareMathOperator{\Exp}{Exp}
\DeclareMathOperator{\Geom}{Geom}
\DeclareMathOperator{\Ber}{Ber}
\DeclareMathOperator{\hor}{hor}
\DeclareMathOperator{\ver}{ver}
\DeclareMathOperator{\N}{\mathbb{N}}

\DeclareMathOperator{\Prob}{\bbP}
\renewcommand{\P}{\Prob}
\DeclareMathOperator{\E}{\bbE}
\def\e{\varepsilon}



\newcommand{\prob}{\sP}
\newcommand{\power}{\sS}
\newcommand{\tie}{\mathfrak{t}}

\newcommand{\RR}{\mathbb{R}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\CC}{\mathbb{C}}

\DeclareMathOperator{\supp}{supp }

\newcommand{\given}{\, | \,}
\newcommand{\Given}{\, \Bigm| \,}
\newcommand\mb[1]{\mathbf{#1}}
\newcommand\mc[1]{\mathcal{#1}}
\newcommand*\mean[1]{\overline{#1}}
\newcommand\eqd{\mathrel{\stackrel{\makebox[0pt]{\mbox{\normalfont\tiny d}}}{=}}}


\newcommand\abullet{{\scaleobj{0.6}{\bullet}}}  %%%% smaller bullet to use inside functions 
\newcommand\bbullet{{\raisebox{0.5pt}{\scaleobj{0.6}{\bullet}}}} %% looks good for paths x_\bbullet 
\newcommand\brbullet{{\raisebox{-1pt}{\scaleobj{0.5}{\bullet}}}} %%  for subscript paths x_\brbullet   need negative raise 
\newcommand\cbullet{{\raisebox{1pt}{\scaleobj{0.6}{\bullet}}}}   %% looks good on Busemann process \Bus^\cbullet  as a subscript  


\DeclareMathOperator*{\argmin}{arg\,min}


\newcommand\aabullet{{\raisebox{1.3pt}{\hspace{0.6pt}\scaleobj{0.55}{\bullet}\hspace{0.75pt}}}}  %%%% smaller bullet to use inside functions, needed to raise it a little and put space around 



\newcommand\eps{\varepsilon}

\newcommand\Z{\mathbb{Z}}
\newcommand\Znonneg{\mathbb{Z}_+}  % The non-negative integers
\newcommand\R{\mathbb{R}}
\newcommand\Rnonneg{\mathbb{R}_+}  % The non-negative real numbers



\font \mymathbb = bbold10 at 11pt
\newcommand\one{\mbox{\mymathbb{1}}}

\DeclareMathOperator*{\Pesssup}{\mathbb{P}-ess\,sup}
\DeclareMathOperator*{\Pessinf}{\mathbb{P}-ess\,inf}

\newcommand\range{\mathcal{R}}  % The set of steps R
\newcommand\rangeA{\mathcal{R}_{\sA}}
\newcommand\Rgroup{\mathcal{G}}  % The additive group generated by the set of steps
\newcommand\RgroupA{\mathcal{G}_{\sA}}
\newcommand\stRgroupA{\overline{\mathcal{G}}_{\sA}}
\newcommand\Rsemi{\mathcal{G}^+} % additive semi-group generated by set of steps
\newcommand\RsemiA{\mathcal{G}_{\sA}^+}
%\newcommand\RposSpan{\mathcal{C}_+} % \sum_{z \in R} a_z z where each a_z \geq 0  
\newcommand\Dn[1]{D_{#1}}  % set of points reachable from the origin in exactly #1 steps
\newcommand\DnA[1]{D_{#1}(\rangeA)}

\newcommand\subspaceA{W_{\sA}}  % The linear subspace of R^d generated by the steps on the face \sA 
\newcommand\subspaceC{W_{\cone}}

\newcommand\maxz{R} % \max_{z \in \range} \abs{z \cdot \uhat}_1
\newcommand\Lt[1]{L_{#1}}  % Points v such that t\ppShapeUnr{\beta}(\xi) \leq v \cdot \uhat \leq t\ppShapeUnr{\beta}(\xi) + \maxz

\newcommand\Uset{\mc{U}}  % convex hull of R
\newcommand\UsetA{\mc{U}_\sA}  % The set \Uset \cap \sA
\newcommand\cone{\mc{C}}  % the cone: \sum_{z \in \range} b_z z  where each b_z \in \R_+

\newcommand\facetUnr[1]{\mc{F}_{#1}^\beta}  % the set of L1 norm 1 directions dual to #1 in the unrestricted duality
\newcommand\facetRes[1]{\Uset_{#1}^\beta}  % the set of directions dual to #1 in the restricted duality (the restricted point-to-line shape(#1) is assumed to be 0.
\newcommand\facetResZero[1]{\Uset_{#1}^\infty}

\newcommand\BHctb{\mc{B}\mc{H}} % countable set of arbitrary (\beta, h) pairs
\newcommand\Bctb{\mc{B}} % countable dense subset of betas
\newcommand\Hctb[1]{\mc{H}^{#1}}  % countable dense subset of tilts for a particular beta
\newcommand\HctbA[1]{\mc{H}_{\sA}^{#1}}  % countable dense subset of tilts for a particular beta

\newcommand\DctbA{\mc{D}_{\sA}} % countable set of pairs (\beta, m) for the face \sA
\newcommand\DctbC{\mc{D}_{\cone}}
\newcommand\DctbCbar{\mc{D}_{\overline\cone}}
\newcommand\Dctb{\mc{D}}


\newcommand\Omegahat{\widehat{\Omega}}  % the enlarged space 
\newcommand\OmegahatA{\widehat{\Omega}_{\sA}}  % the enlarged space for a particular face
\newcommand\omegahat{\widehat{\omega}}

\DeclareMathOperator{\id}{id}
\DeclareMathOperator\coc{coc}
\DeclareMathOperator\dir{dir}
\DeclareMathOperator{\reg}{reg}
\newcommand\OmegaCoc{\widehat{\Omega}_{\coc}}  % the full probability event contained in \Omegahat on which cocycle, recovery hold 
\newcommand\OmegaCocA{\widehat{\Omega}_{\sA, \coc}}  % the full probability event contained in \OmegahatA on which cocycle, recovery hold on the face \sA
\newcommand\OmegaDir{\Omega_{\dir}}  % the full measure event (inheriting the properties of \OmegaCoc) on which the constructed semi-infinite path measures are consistent and directed 
%\newcommand\OmegaDirA{\Omega_{\sA, \dir}} % the full measure event (inheriting the properties of \OmegaCocA) on which the constructed semi-infinite path measures are consistent and directed on the face \sA
\newcommand\OmegaReg{\Omega_{\reg}} % the full measure event where we have regular conditional distributions to take slices to get back to the original space

\newcommand\wProj{\pi_{\Omega}(\omegahat)}  % The projection of \omegahat to the original space


\newcommand\Sig{\mfS} % Borel sigma-algebra on the space
\newcommand\Sighat{\widehat{\mfS}}  % Borel sigma-algebra on the enlarged space
\newcommand\SighatA{\widehat{\mfS}_{\sA}}  % Borel sigma-algebra on the enlarged space for face \sA
\newcommand\invSig{\mc{I}} % Sigma-algebra of T-invariant events
\newcommand\wSig{\mathfrak{S}}  % No longer used:  Sigma-algebra generated by the omega-weights


\newcommand\meanVec{\mathfrak{h}}  % The mean vector of the restricted-length Busemann (only unique if the R set spans R^d)
\newcommand\meanVecUnr{\hbar}  % Mean vector of unrestricted length Busemann


\newcommand\PathsNStep[2]{\mathbb{X}_{#1}^{#2}}  % The set of all paths of length #2 starting at #1

\newcommand\PathsPtPUnr[2]{\mathbb{X}_{#1, #2}} % Set of all paths from #1 to #2.  May be any length, and may revisit #2 (like in the Green's function definition.)

\newcommand\PathsLvKilled[2]{\overline{\mathbb{X}}_{#1, (#2)}}  % The set of all unrestricted length paths starting at #1 until the first time they reach or exceed level n.
\newcommand\PathsNearLvn[3]{\overline{\mathbb{X}}_{#1, (#2)}^{#3}} % The set of all unrestricted length paths starting at #1 until the first time they reach a point v which is close to level n (relative to xi and uhat)

\newcommand\PathsPtPKilledRes[3]{\overline{\mathbb{X}}_{#1, #2}^{#3} } % Set of all paths from #1 to the first time it hits #2 in #3 steps, restricted length
\newcommand\PathsPtPKilled[2]{\overline{\mathbb{X}}_{#1, #2} } % Set of all paths from #1 to the first time it hits #2, unrestricted length

\newcommand\PathsPtPRes[3]{\mathbb{X}_{#1, #2}^{#3}}  % Set of all paths from #1 to #2 that take #3 steps
\newcommand\PathsPtPResKM[4]{\mathbb{X}_{#1, #2}^{#3, #4}}  % Set of all paths from #1 at time #3 to #2 at time #4

\newcommand\PathsSemiInf[1]{\mathbb{X}_{#1}} % Set of all semi-infinite paths starting at #1


\newcommand\Cocycles{\mathcal{K}}  % The space of shift-covariant space-time cocycles
\newcommand\cenCocycles{\mathcal{K}_{0}}  % The space of shift-covariant centered space-time cocycles
\DeclareMathOperator{\spacetime}{st}  % indicates space-time cocycles, rather than space-only
\newcommand\SpaceTimeCocycles{\mathcal{K}_{\spacetime}}  % The space of shift-covariant space-only cocycles
\newcommand\cenSpaceTimeCocycles{\mathcal{K}_{\spacetime,0}}  % The space of shift-covariant centered space-only cocycles


\newcommand\faces{\mathbb{A}} % the set of all non-zero faces of \cone

\newcommand\T{T} % original shifts
\newcommand\That{\widehat{T}} % shifts on enlarged space
\newcommand\ThatA{\widehat{T}'} % shifts on the enlarged space for a face \sA

%\newcommand\ehat{\widehat{e}}  % The vector <1, 1, ..., 1> \in \RR^d
\newcommand\uhat{\widehat{u}}  % vector defining the level sets
\newcommand\orig{\mathbf{0}}  % The vector <0, 0, ..., 0> \in \RR^d

\newcommand\classL{\mc{L}}  % The class L for the potential function
\newcommand\pote{V}  % The potential function 

\newcommand\stoppt[1]{\tau_{#1}}  % stopping time first time we reach point #1
\newcommand\stoplv[1]{\sigma_{#1}}  % stopping time first time we reach level >= #1 

\DeclareMathOperator{\rwP}{P} % classical random walk starting at x giving equal probabilities to each increment in R
\DeclareMathOperator{\rwE}{E} % " "

%\newcommand\bbP{\mathbb{P}}  % product measure
%\newcommand\bbE{\mathbb{E}}  %  " " 

\newcommand\bbUn{\mathbb{U}_n}  % discrete uniform on {1, 2, \ldots, n}
\newcommand\bbPU{\overline\bbP}  %\bbP\otimes\bbU
\newcommand\bbPn{\mathbb{P}_n}  %  the product measure times the discrete uniform on {1, 2, ..., n}
\newcommand\bbEn{\mathbb{E}_n}  %  " "
\newcommand\bbEU{\overline\bbE}  %  " "

\newcommand\bbPhat{\widehat{\mathbb{P}}} % subsequential limit
\newcommand\bbEhat{\widehat{\mathbb{E}}} % "

\newcommand\bfPn{\mathbf{P}_n}  % laws of $(\omega, B_n......) from which we extract the subsequential limit
\newcommand\bfPnk{\mathbf{P}_{n_k}}  % "
\newcommand\bfEnk{\mathbf{E}_{n_k}}  % "
\newcommand\bfPne{\mathbf{P}_{n,\e}}  % laws of $(\omega, B_{n,\e}......) from which we extract the subsequential limit
\newcommand\bfPs[1]{\mathbf{P}_{#1}} % "
\newcommand\bfEs[1]{\mathbf{E}_{#1}} % "
\newcommand\bfPe{\mathbf{P}_{\e}} % after we take weak subsequential limit in n, get this law for each \e
\newcommand\bfEe{\mathbf{E}_{\e}} % "

\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\ext}{ext} % extreme 


%%%%Gibbs measures sets
\def\DLR{\mathrm{DLR}}
\newcommand{\siDLR}{\overrightarrow{\DLR}}
\newcommand{\biDLR}{\overleftrightarrow{\DLR}}
 
\newcommand\superDiffRes[1]{\partial \Lambda_{\res}^{#1}}  % subdifferential of the restricted length point-to-point limiting free energy
\newcommand\superDiffUnr[1]{\partial \Lambda^{#1}}  % subdifferential of the unrestricted length point-to-point limiting free energy
\newcommand\superDiffResA[1]{\partial \Lambda_{\res, \sA}^{#1}} % subdifferential of the restricted length point-to-point limiting free energy on the face \sA
\newcommand\superDiffUnrA[1]{\partial \Lambda_{\sA}^{#1}} % subdifferential of the unrestricted length point-to-point limiting free energy on the face \sA

\DeclareMathOperator{\pp}{pp} % point-to-point quantity
\DeclareMathOperator{\pl}{pl}  % indicates point-to-level quantity
\DeclareMathOperator{\lsc}{lsc}  % lower semi-continuous regularization
\DeclareMathOperator{\usc}{usc}  % upper semi-continuous regularization
\DeclareMathOperator{\res}{res}  % used to indicate a restricted-length quantity 
\DeclareMathOperator{\cont}{cont}  % continuous extension

\newcommand\ppShapeRes[1]{\Lambda^{#1}_{\res}}  % Point-to-Point limiting free energy, restricted length
\newcommand\ppShapeResA[1]{\Lambda^{#1}_{\sA, \res}}  % " restricted to face \sA
\newcommand\ppShapeResU[1]{\Lambda^{#1}_{\sU', \res}}  % " restricted to face \sU'
\newcommand\ppShapeUnr[1]{\Lambda^{#1}} % Point-to-Point limiting free energy, unrestricted length
\newcommand\ppShapeUnrA[1]{\Lambda^{#1}_{\sA}} % " restricted to face \sA
\newcommand\plShapeRes[1]{\Lambda_{\res, \pl}^{#1}}  % N-step restricted length limiting free energy
\newcommand\plShapeUnr[1]{\Lambda_{\pl}^{#1}}  % point-to-level unrestricted limiting free energy 




\newcommand\prtres[4]{Z_{#1, #2, #3}^{#4}}  % partition function from #1 to #2 in #3 steps, with parameters #4 
\newcommand\prtnstep[3]{Z_{#1, #2}^{#3}}  % partition function from #1 with paths of length #2, parameters #3

\newcommand\prtunr[3]{Z_{#1, #2}^{#3}}  %  partition function from #1 to #2 (unrestricted length) with parameters #3
\newcommand\prtlevn[3]{Z_{#1, (#2)}^{#3}}  % partition function from #1 to level #2 with parameters #3


\newcommand\freeres[4]{F_{#1, #2, #3}^{#4}}  % restricted-length pre-limit free energy.  Goes from #1 to #2 in #3 steps with parameters #4
\newcommand\freeunr[3]{F_{#1, #2}^{#3}}  % unrestricted-length pre-limit free energy.  Goes from #1 to #2 with parameters #3

\newcommand\freenstep[3]{F_{#1, #2}^{#3}} % n-step (restricted-length) free energy.  Go from #1 with #2 steps, parameters #3
\newcommand\freelevn[3]{F_{#1, (#2)}^{#3}} % Unrestricted-length equivalent of ``point to level'' free energy.  Go from #1 to level #2 (or a point near level #2), parameters #3


\newcommand\convMeas{\sM} % the convex set of semi-infinite path measures which satisfy consistency
%\newcommand\convMeasA{\sM^{\beta,\w}_{x,\sA}}  % same with measures defined on the face \sA
\newcommand\convMeasA{\siDLR_{x,\sA}^{\beta,\w}}  % same with measures defined on the face \sA
\newcommand\Qres[4]{\textup{Q}_{#1, #2, #3}^{#4}} % Finite path measure, restricted length. Goes from #1 to #2 in #3 steps with parameters #4
\newcommand\Qunr[3]{\textup{Q}_{#1, #2}^{#3}} % Finite path measure, unrestricted length. Goes from #1 to #2 with parameters #3
\newcommand\QnStep[3]{\textup{Q}_{#1, #2}^{#3}} % N step, restricted length. Goes from #1 for #2 steps with parameters #3
\newcommand\Qlv[3]{\textup{Q}_{#1, (#2)}^{#3}} % Point-to-level, unrestricted length. Goes from #1 to level #2 with parameters #3


\newcommand\Qinf[2]{\textup{Q}_{#1}^{#2}} % Infinite path measure starting at #1
\newcommand\greens{g}  % Green's function
\newcommand\Qtil[2]{\widetilde{\textup{Q}}_{#1}^{#2}} % Alternate path measure based on Green's function


 
\newcommand\psgres[3]{G_{#1, #2, #3}} % passage time from #1 to #2 in #3 steps
\newcommand\psgLv[3]{G_{#1, (#2)}^{#3}} % unrestricted length passage time from #1 to level #2, with face #3
\newcommand\psgUnr[2]{G_{#1, #2}} % passage time from #1 to #2, unrestricted length


\newcommand\Bn[2]{B_{#1}^{#2}}  % pre-limit Busemann 

\newcommand\BNn[1]{B_{N_n}^{#1}}  % Uses N_n chosen uniformly from 1, ..., n
\newcommand\BUn[1]{B_{U_n}^{#1}}  % Uses U_n chosen uniformly from 1 to n
\newcommand\BUne[1]{B_{U_n,\e}^{#1}}  % Uses U_n chosen uniformly from 1 to n, but with \e margin

\newcommand\B[1]{B^{#1}}  % post-limit Busemann in our construction

\newcommand\Btil[1]{\widetilde{B}^{#1}}  % B conditioned on the sigma algebra generated by omega weights

\newcommand\hVec{\mathbf{h}}  % mean -h(B) for a recovering cocycle B
\newcommand\mVec{\mathbf{m}}  % mean m(B) for a recovering cocycle B
\newcommand\m{m}  % the parameter m that is used to construct the cocycles








\usepackage{xargs}
\addtolength\marginparwidth{+.1in}

\usepackage[colorinlistoftodos,prependcaption,textsize=footnotesize]{todonotes}
\newcommandx{\addmath}[2][1=]{\todo[linecolor=red,backgroundcolor=red!25,bordercolor=red,#1]{#2}}
\newcommandx{\fixtext}[2][1=]{\todo[linecolor=blue,backgroundcolor=blue!25,bordercolor=blue,#1]{#2}}
\newcommandx{\note}[2][1=]{\todo[linecolor=yellow,backgroundcolor=yellow!25,bordercolor=yellow,#1]{#2}}
\def\seannote#1{{\color{my-green}{(S: #1)}}}
\def\chrisnote#1{{\color{blue}{(C: #1)}}}
\def\firasnote#1{{\color{orange}{(F: #1)}}}
\def\mathnote#1{{\color{red}{(#1)}}}
\def\thesisnote#1{{\color{brown}{#1}}}

%\newcommand\aUset{\sV^{\,\w}} %The set of directions on which non-coalescence holds
%\newcommand\gpp{g} %The shape function without pp subscript 
%\newcommand\dgpp[1]{\widecheck{g}_{\text{pp}}^{#1}} %The shape function
%\newcommand\T{T} %The shift, T
%\newcommand\cid{\xi_*} %The competition interface random variable
%\newcommand\adir{\zeta} 
%\newcommand\wchk[1]{\widecheck{\omega}^{#1}} %Dual weights
%\DeclareMathOperator{\Exit}{Exit}

%Busemann functions
%\newcommand\B[1]{B^{#1}} %The Busemann function
%\newcommand\BBbar[1]{{\overline B}^{#1}} %The Busemann function
%\newcommand\Ubar{\overline U} %The Busemann function
%\newcommand\dB[1]{u^{#1}} %The Busemann function
%\newcommand\dBbar[1]{\overline{u}^{#1}} %The Busemann function

%Geodesics
%\newcommand\geo[3]{\boldsymbol{\gamma}_{#1}^{\,#2,#3}} %Geodesic. Arguments are 1.) the index, 2.) the starting point, 3.) the direction
%\newcommand\geobar[3]{{\overline{\boldsymbol{\gamma}}}_{#1}^{\,#2,#3}} %Geodesic. Arguments are 1.) the index, 2.) the starting point, 3.) the direction
%\newcommand\geod[1]{\pi_{#1}} %A generic geodesic without a root or direction. The argument is the index.
%\newcommand\geod[1]{\boldsymbol{\gamma }_{#1}} %A generic geodesic without a root or direction. The argument is the index.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%Environments
\newtheorem{mainCounter}{MainCounter}[section]
\newtheorem{lemma}[mainCounter]{Lemma}
\newtheorem{theorem}[mainCounter]{Theorem}
\newtheorem{itheorem}[mainCounter]{Informal Theorem}
\newtheorem{prop}[mainCounter]{Proposition}
\newtheorem{cor}[mainCounter]{Corollary}
\numberwithin{equation}{section}
\newtheorem{definition}[mainCounter]{Definition}
\newtheorem{condition}[mainCounter]{Condition}

%Put the figures on the same counter as theorems


\theoremstyle{remark}
\newtheorem{remark}[mainCounter]{Remark}
\AtBeginEnvironment{remark}{%
  \pushQED{\qed}\renewcommand{\qedsymbol}{$\triangle$}%
}
\AtEndEnvironment{remark}{\popQED\endremark}
\newtheorem{example}[mainCounter]{Example}
\AtBeginEnvironment{example}{%
  \pushQED{\qed}\renewcommand{\qedsymbol}{$\triangle$}%
}
\AtEndEnvironment{example}{\popQED\endremark}

%\newtheorem{comment}[mainCounter]{Comment}

\allowdisplaybreaks[1]
% Change the subfigure numbering style to Roman numerals
\captionsetup[subfigure]{labelformat=simple, labelsep=colon} % Format subfigure labels
\renewcommand{\thesubfigure}{\Alph{subfigure}} % Add parentheses around the label

